"Does 4-4-2 exist?" -- An Analytics Approach to Understand and Classify Football Team Formations in Single Match Situations

The chances to win a football match can be significantly increased if the right tactic is chosen and the behavior of the opposite team is well anticipated. For this reason, every professional football club employs a team of game analysts. However, at present game performance analysis is done manually and therefore highly time-consuming. Consequently, automated tools to support the analysis process are required. In this context, one of the main tasks is to summarize team formations by patterns such as 4-4-2. In this paper, we introduce an analytics approach that automatically classifies and visualizes the team formation based on the players' position data. We focus on single match situations instead of complete halftimes or matches to provide a more detailed analysis. A detailed analysis of individual match situations depending on ball possession and match segment length is provided. For this purpose, a visual summary is utilized that summarizes the team formation in a match segment. An expert annotation study is conducted that demonstrates 1) the complexity of the task and 2) the usefulness of the visualization of single situations to understand team formations. The suggested classification approach outperforms existing methods for formation classification. In particular, our approach gives insights about the shortcomings of using patterns like 4-4-2 to describe team formations.

==> fig_cms.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0.4cm 0.5cm 0.4cm 0.4cm},clip]{graphics/breakingnews_wd_PERSONS-relevant_TEST_text_spaCy_max_at-100_plot.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}  
        \centering 
        \includegraphics[width=\textwidth,trim={0.4cm 0.5cm 0.4cm 0.4cm},clip]{graphics/breakingnews_wd_PERSONS-relevant_TEST_text_spaCy_max_at-25_plot.pdf} 
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0.4cm 0.5cm 0.4cm 0.4cm},clip]{graphics/breakingnews_wd_PLACES-relevant_TEST-outdoor_text_spaCy_quantil10_at-25_plot.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}  
        \centering 
        \includegraphics[width=\textwidth,trim={0.4cm 0.5cm 0.4cm 0.4cm},clip]{graphics/breakingnews_wd_EVENTS-relevant_TEST_text_spaCy_quantil10_at-25_plot.pdf} 
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}  
        \centering 
        \includegraphics[width=\textwidth,trim={0.4cm 0.5cm 0.4cm 0.4cm},clip]{graphics/breakingnews_document_text_TEST_text_max_at-25_plot.pdf} 
    \end{subfigure}
    \caption{Sorted \emph{Cross-modal Similarity} values for for all entity types using different modification techniques according to~Section~\ref{sec:datasets} evaluated on the \emph{BeakingFakeNews} dataset. Best viewed in color.} %The decision threshold~(red) is used for classification. Best viewed in color. The green area represents the Top-25\% documents with respect to the similarity.}
    \label{fig:cms}
\end{figure*}

==> tab_topk-template-fsim.tex <==
\begin{table}[]
    \caption{mean similarity for the top-$k$ closest formations}
    \label{tab:topk-template-fsim}
    \begin{tabular}{lllll}
                          $F_n$ & top-1  & top-2  & top-3 & top-4 \\ \hline
    \multicolumn{1}{l|}{ 4-4-2 }  & 0.728  & 0.715  & 0.703  & 0.692 \\
    \multicolumn{1}{l|}{ 4-3-3 }  & 0.768  & 0.676  & 0.639  & 0.614 \\
    \multicolumn{1}{l|}{ 4-1-4-1 }  & 0.934  & 0.926  & 0.902  & 0.829 \\
    \multicolumn{1}{l|}{ 4-2-3-1 }  & 0.744  & 0.654  & 0.606  & 0.581 \\
    \multicolumn{1}{l|}{ 5-4-1 }  & 0.918  & 0.845  & 0.803  & 0.772 \\
    \multicolumn{1}{l|}{ 4-5-1 }  & 0.934  & 0.860  & 0.813  & 0.779 \\
    \multicolumn{1}{l|}{ 5-3-2 }  & 0.683  & 0.680  & 0.674  & 0.655 \\
    \multicolumn{1}{l|}{ 4-2-4 }  & 0.744  & 0.723  & 0.677  & 0.642 \\
    \multicolumn{1}{l|}{ 3-5-2 }  & 0.584  & 0.562  & 0.529  & 0.513 \\
    \multicolumn{1}{l|}{ 4-3-2-1 }  & 0.852  & 0.819  & 0.803  & 0.794 \\
    \multicolumn{1}{l|}{ 3-4-3 }  & 0.677  & 0.631  & 0.600  & 0.558 \\
    \multicolumn{1}{l|}{ 3-3-4 }  & 0.677  & 0.631  & 0.575  & 0.536 \\
    \hline
    Mean & 0.770 & 0.727 & 0.694 & 0.664
    \end{tabular}
\end{table}
